CoTracker: It is Better to Track Together

We introduce CoTracker, a transformer-based model that tracks a large number of 2D points in long video sequences. Differently from most existing approaches that track points independently, CoTracker tracks them jointly, accounting for their dependencies. We show that joint tracking significantly improves tracking accuracy and robustness, and allows CoTracker to track occluded points and points outside of the camera view. We also introduce several innovations for this class of trackers, including using token proxies that significantly improve memory efficiency and allow CoTracker to track 70k points jointly and simultaneously at inference on a single GPU. CoTracker is an online algorithm that operates causally on short windows. However, it is trained utilizing unrolled windows as a recurrent network, maintaining tracks for long periods of time even when points are occluded or leave the field of view. Quantitatively, CoTracker substantially outperforms prior trackers on standard point-tracking benchmarks.

==> accuracy_grid_size_figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth,trim={0.8cm 0 0 0}]{figures/accuracy_grid_size_figure.pdf}
    \caption{\textbf{Number of points}. \nk{todo: remove it} We track queried points from TAP-Vid-DAVIS together with $N$ additional points sampled on the first frame. Adding 16-25 points is best, while more points overwhelm tracking the interest points.}
    \label{fig:my_label}
\end{figure}



==> figure_ims.tex <==
\begin{figure}[t]    
  \centering
  \includegraphics[width=\textwidth]{figures/figure_ims.pdf}
  \caption{\textbf{Qualitative Examples}.
  CoTracker predicts the tracks for an arbitrary selection of points in long videos. In these examples from DAVIS~\cite{pont20172017}, the points are selected on an object of interest, but any point can be tracked. Here, we compensate for camera motion by using predicted background tracks and visualize the object tracks with colored lines.}
  \label{fig:figure_ims}
  % (see \cref{tab:tab_joint_tracking_ablation}).}%
\end{figure}


==> plot_efficiency.tex <==

\begin{figure}{h}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/plot_efficiency.pdf}
    \caption{\textbf{Efficiency}. We track queried points from the TAP-Vid-DAVIS~\cite{tapvid} dataset together with $N^2$ points sampled on the first frame, where $N$ is the grid size. When tracking $<800$ points queried at different frames, \method is more efficient than PIPs~\cite{pips} and RAFT~\cite{raft}.}%
    \label{fig:efficiency}
\end{figure}



==> plot_joint_individual.tex <==
\begin{figure}[h!]
    % \centering
    \includegraphics[width=\textwidth]{figures/plot_joint_individual.pdf}
    \caption{\textbf{Single point vs. joint tracking.} We qualitatively compare tracking individual points (top
    row) to tracking all points together (bottom). Background points are colored cyan while foreground
    points are magenta. We find that single-point tracking leads to background points following the object
    motion, as the model cannot reason well about the global context of the video (cyan points in later
    frames). Tracking points together results in better tracks for foreground and background points.}
\end{figure}



==> tabs/tab_ablation_unrolled.tex <==
%\setlength\tabcolsep{.4em}
\begin{table}[t]
\centering
\footnotesize

\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{Unrolled Training} & \multicolumn{3}{c}{DAVIS First} \\
\cmidrule(lr){2-4}
& AJ \ua& \davg \ua& OA \ua\\ 
\midrule
% \midrule
\xmark  & 44.6  & 60.5  & 75.3 \\
\cmark & \textbf{62.2} & \textbf{75.7} & \textbf{89.3 }\\
\bottomrule
\end{tabular}
\caption{ \textbf{Unrolled training.} \method is built for sliding window predictions. Using them during training is important.
\nk{explain details}
}\label{tab:tab_unrolling}
\end{table}






==> tabs/tab_comparison_dr.tex <==
\begin{table}[t]
\centering
\small

\label{tab:tab_comparison_dr}
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Dynamic Replica}\\
\cmidrule(lr){2-4}
                                & \davg\ua & \davgvis\ua   & \davgocc\ua  \\
\midrule
TAP-Net~\cite{tapvid}           & 45.5 & 53.3 & 20.0 \\
PIPs ~\cite{harley22particle}            & 41.0 & 47.1 & 21.0 \\

PIPs++~\cite{zheng2023pointodyssey}                & 55.5 & 64.0 & 28.5 \\
TAPIR~\cite{doersch2023tapir} & 56.8 & 66.1 & 27.2 \\
\midrule
CoTracker (Ours)                  & \textbf{61.6} & \textbf{68.9 } & \textbf{37.6} \\
\bottomrule
\end{tabular}
\caption{
\textbf{Dynamic Replica}.}%
\end{table}






==> tabs/tab_dino_ablation.tex <==
%\setlength\tabcolsep{.4em}
\begin{table}[t]
\centering
\footnotesize
\caption{  \textbf{Feature network}. Replacing the image encoder with a frozen pre-trained Vision Transformer decreases the performance. }\label{tab:dino_ablation}
\begin{tabular}{ lcccccc }
\toprule
 \multirow{2}{*}{Feature Network}  & \multicolumn{3}{c}{DAVIS First} & \multicolumn{2}{c}{BADJA} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-6}
             & AJ            & \! \! \! $< \delta^x_{avg}$\! & OA            & \! \! seg-based\! \! & \! \! $< \delta^{3px}$ \! \! \\
\midrule
\textbf{CNN} & \textbf{51.2} & \textbf{68.5}                 & \textbf{85.2} & 65.5                 & \textbf{15.4}                \\
DINOv2       & 38.8          & 56.2                          & 83.6          & \textbf{67.3}        & 9.1                          \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/tab_space_time_ablation_old.tex <==
\setlength\tabcolsep{.5em}
\begin{table}[t]
\centering

\setlength{\tabcolsep}{4pt}
\begin{tabular}{c cc c>{\centering}p{1.5cm} ccc}
\toprule
&\multicolumn{2}{c}{Attention} & \multicolumn{2}{c}{Points} & \multicolumn{3}{c}{DAVIS First} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-8}
   &time   & joint  & target & support                             & AJ \ua                 &  \davg\ua & OA \ua         \\
\midrule
(a)&\cmark & \xmark & single & ---    &           58.3                      &        71.5   &  86.4               \\

(b)&\cmark & \cmark & single & ---                       &        41.1   &    62.9     & 75.1              \\

(c)&\cmark & \cmark & single & glob. $9\ctimes9$                   & 56.8                  &  71.2              & 85.8          \\
(d)&\cmark & \cmark & single & SIFT $8\ctimes8$                    & 57.4                  &  72.1              & 85.8          \\
(e)&\cmark & \cmark & single & loc.~$10\ctimes10$                  & 60.4                  &  75.2              & 87.5          \\
(f)&\cmark & \cmark & single & glob. $5\ctimes5$ +loc. $8\ctimes8$ & \textbf{62.2}         &  \textbf{75.7}     & \textbf{89.3} \\ 

\midrule
(g)&\cmark & \cmark & all    & ---                                 & 57.6                  &  73.2              & 86.1          \\
(h)&\cmark & \cmark & all    & glob. $5\ctimes5$                   & 60.5                  &  \textbf{75.8}     & 87.6          \\
(i)&\cmark & \cmark & all    & SIFT $8\ctimes8$                    & \textbf{60.7}         &  75.7              & \textbf{88.1} \\
\bottomrule
\end{tabular}
\caption{\nk{We need to simplify this table. SEE THE NEW TABLE BELOW. } \textbf{Importance of joint tracking}.
We compare models pre-trained with time and cross-track attention, while tracking single or multiple target points, and using additional support points.
}%
\label{tab:tab_joint_tracking_ablation}
%
\end{table}




==> tabs/tab_suppl_train_data.tex <==
%\setlength\tabcolsep{.4em}
\begin{table*}[t]
\centering
\footnotesize
\caption{  \textbf{Training data}.  }\label{tab:tab_train_data_comparison}
\begin{tabular}{ llccccccccc }
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Training data}  & \multicolumn{3}{c}{TAP-Vid Davis} & \multicolumn{3}{c}{TAP-Vid Kinetics} & \multicolumn{2}{c}{BADJA} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
& &  AJ & \!\!\!$< \delta^x_{avg}$\! & OA  & AJ & \!\!\!$< \delta^x_{avg}$ & OA & \!\!seg-based\!\! & \!\!3px acc\!\! \\
\midrule

PIPs~\cite{pips} & Flying things++ & 42.2 & 64.8 & 77.7 & 31.7 & 53.7 & 72.9 & 61.9 & 13.5 \\

PIPs~\cite{pips} & TAP-Vid-Kubric  & 43.8 & 66.5 & 77.4 & 32.7 & 55.1 & 72.9 & 64.0 & 14.7 \\
PIPs~\cite{pips} & Dynamic Replica   & 39.7 & 61.5 &  &  &  & & 59.6 &  12.4 \\

\method (Ours)\!\!\! & TAP-Vid-Kubric              & \textbf{51.2} & \textbf{68.5} & \textbf{85.2} & \textbf{43.3} & \textbf{61.4} & \textbf{83.3} & \textbf{65.5} & \textbf{15.4} \\
\method (Ours)\!\!\! & Dynamic Replica    & & & & & & &      62.8    & 16.6 \\

\bottomrule
\end{tabular}

\end{table*}



==> tabs/tab_train_data_comparison.tex <==
%\setlength\tabcolsep{.4em}
\begin{table}[t]
\centering
\footnotesize
\caption{  \textbf{Training data}. For a fair comparison, we train PIPs on Kubric which improves performance.  }\label{tab:tab_train_data_comparison}
\begin{tabular}{ llcccccc }
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Training data}  & \multicolumn{3}{c}{DAVIS First}  \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-7}
& &  AJ & \!\!\!$\davg$\! & OA \\
\midrule
% \midrule
PIPs~\cite{pips} & Flying things++ & 42.2 & 64.8 & 77.7 \\
 
PIPs~\cite{pips} & TAP-Vid-Kubric  & 43.8 & 66.5 & 77.4 \\

\method (Ours)\!\!\! & TAP-Vid-Kubric    & \textbf{60.6} & \textbf{75.4} & \textbf{89.3 } \\

\bottomrule
\end{tabular}

\end{table}


==> tabs/tab_window_size.tex <==
%\setlength\tabcolsep{.4em}
\begin{table}[t]
\centering
\footnotesize
\caption{ \textbf{Training sliding window size}. We train and evaluate \method with the varying window lengths. As the training data only contains sequences of length 24, larger window sizes are difficult to train.}%
\label{tab:window_size}
\begin{tabular}{ lccccc }
\toprule
\multirow{2}{*}{Window size} & \multicolumn{3}{c}{DAVIS First} & \multicolumn{2}{c}{BADJA} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-6}
           & AJ            & $< \delta^x_{avg}$ & OA            & seg-based     & \! \! $< \delta^{3px}$ \! \! \\ \midrule
4          & 57.9          & 73.2               & 87.0          & 64.6          & 18.2                         \\
\textbf{8} & \textbf{60.6} & \textbf{75.4}      & \textbf{89.3} & 63.6          & 18.0                         \\
12         & 58.8          & \textbf{75.4}      & 87.6          & \textbf{65.1} & 17.7                         \\
16         & 57.8          & 75.2               & 86.7          & 64.1          & \textbf{18.4}                \\
20         & 57.3          & 74.0               & 85.9          & 64.9          & 18.3                         \\ \bottomrule
\end{tabular}
\end{table}


